Measurement of the $\Omega_c^0$ lifetime at Belle II

We report on a measurement of the $\Omega_c^0$ lifetime using $\Omega_c^0 \to \Omega^-\pi^+$ decays reconstructed in $e^+e^-\to c\bar{c}$ data collected by the Belle II experiment and corresponding to $207~{\rm fb^{-1}}$ of integrated luminosity. The result, $\rm\tau(\Omega_c^0)=243\pm48( stat)\pm11(syst)~fs$, agrees with recent measurements indicating that the $\Omega_c^0$ is not the shortest-lived weakly decaying charmed baryon.

==> Makefile <==
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# A few changes by Angelo Di Canto on 2018-08-21
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = draft

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = BELLE2-PUB-DRAFT-2021-002

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

FIGEXT = .pdf
MAINEXT= .pdf

BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)

BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl

MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' $(MAIN)-prl.tex > $(MAIN)-count.tex
BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf $(MAIN)-count* 

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.sty)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(TARGET)*.pdf $(MAIN)$(MAINEXT) $(MAIN)-prl$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout:
	rm $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN)-PRLstyle$(MAINEXT)

# make arxiv tarball
arxivtgz: $(OUTPUT)
	rm -f $(TARGET)-arxiv.tgz
	tar -czf $(TARGET)-arxiv.tgz $(MAIN).bbl $(SOURCES)

# make the PRL version
prl: 
	$(BUILDCOMMANDPRL)
	cp $(MAIN)-prl$(MAINEXT) $(TARGET)-PRLstyle$(MAINEXT)

# make PRL tarball (can also be used for arxiv)
prltgz: prl
	latexpand --makeatletter --empty-comments --explain --expand-bbl $(MAIN)-prl.bbl -o prlsingle.tex $(MAIN)-prl.tex
	rm -f $(TARGET)-prl.tgz
	tar -czf $(TARGET)-prl.tgz prlsingle.tex figs/*.pdf

# make word count
count: 
	chmod +x wordcount.sh
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo ''
	@echo 'Abstracts should also be ≤ 600 characters'


==> addref <==
#!/usr/bin/env python3
# -*- coding: utf-8 -*-

from urllib.request import urlopen
import sys
import re

# check arguments
if len(sys.argv) != 2:
    print('ERROR: An arXiv or inspire ID has to be given as argument')
    sys.exit(1)

id = sys.argv[1]
bibfile = 'references.bib'

# get bibtex from inspire
if '/' in id:
    query = 'eprint'
elif '.' in id:
    query = 'arxiv'
else:
    query = 'recid'
try:
    bibtex = urlopen(f'https://inspirehep.net/api/literature?q={query}%3A{id}&format=bibtex').read().decode()
except:
    print(f'ERROR: Query for {id} failed.')
    sys.exit(1)
if len(bibtex) == 0:
    print(f'ERROR: Could not get bibtex for {id}.')
    sys.exit(1)

# check whether the entry is already in references.bib
entry = re.compile('@[\w]*{([\S]*),').findall(bibtex)[0]
with open(bibfile) as bib:
    if entry in bib.read():
        print(f'ERROR: {bibfile} already contains the entry {entry}.')
        sys.exit(1)

# add bibtex to references.bib
with open(bibfile, 'a+') as bib:
    bib.write('\n' + bibtex)

print(f'Entry {entry} added to {bibfile} -> \\cite{{{entry}}}')


==> belle2sym.tex <==
%%%%%   Standard symbols for use in Belle II notes and papers. 
%%%%%
%%%%%	C. Hearty	21-Oct-2014		Based on babarsym.tex; authored by D. Hitlin, D. MacFarlane, P. Dauncey, and R. Waldi
%%%%%


\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units (these macros add a small space in front)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nospaceunit}[1]{\ensuremath{\text{#1}}}       
\newcommand{\aunit}[1]{\ensuremath{\text{\,#1}}}       
\newcommand{\unit}[1]{\aunit{#1}\xspace}                   % {kg}   

%%%%%%%%%%%%%%%%%%%% THE NAME OF THE COLLABORATION %%%%
\def\belletwo{Belle~II\xspace}

\newcommand{\CP}{\ensuremath{C\!P}\xspace}
\newcommand{\Acp}{\ensuremath{\mathcal{A}_{\CP}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
%\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle\rm S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle\rm L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\D       {\ensuremath{D}\xspace}
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\part{\xspace}}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^{*+}_s}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}
\def\SixS  {\Y6S}

\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}
\def\Omgc        {\ensuremath{\Omega^0_c}\xspace}
\def\Omg         {\ensuremath{\Omega^-}\xspace}
\def\Lb          {\ensuremath{\Lambda^0}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{{\rm \,km}}\xspace}
\def\m    {\ensuremath{{\rm \,m}}\xspace}
\def\cm   {\ensuremath{{\rm \,cm}}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{{\rm \,mm}}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\nospaceunit{m}}\xspace}%% mu meter 
\def\muma       {\ensuremath{{\,\mu\rm m}^2}\xspace}
\def\nm   {\ensuremath{{\rm \,nm}}\xspace}
\def\fm   {\ensuremath{{\rm \,fm}}\xspace}
\def\nm         {\ensuremath{{\rm \,nm}}\xspace}   %% nanometer
%
\def\barn{\ensuremath{{\rm \,b}}\xspace}
\def\barnhyph{\ensuremath{{\rm -b}}\xspace}
\def\mbarn{\ensuremath{{\rm \,mb}}\xspace}
\def\mbarnhyph{\ensuremath{{\rm -mb}}\xspace}
\def\nb         {\ensuremath{{\rm \,nb}}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{{\rm \,pb}}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second 
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees

\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}

\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    


\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

\newcommand{\stat}{\ensuremath{\,\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\,\mathrm{(syst)}}\xspace}

\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\def\qsq{\ensuremath{q^2}\xspace}


==> pub012-plain.tex <==
%%% Paper:    Omega_c lifetime
%%% Journal:  Physical Review D (L)
%%% Contacts: A. Di Canto, N.K. Nisar
%%% ====================================================================
%%% Use \input{pub012-plain} to insert this material into your latex file.
  \author{F.~Abudin{\'e}n} % 2250
  \author{I.~Adachi} % 2590
% \author{K.~Adamczyk} % 2239
  \author{L.~Aggarwal} % 10083
% \author{P.~Ahlburg} % 2367
  \author{H.~Ahmed} % 11323
% \author{J.~K.~Ahn} % 7423
  \author{H.~Aihara} % 2223
  \author{N.~Akopov} % 9443
  \author{A.~Aloisio} % 2194
% \author{F.~Ameli} % 4683
% \author{L.~Andricek} % 2098
 \author{N.~Anh~Ky} % 2218
 \author{D.~M.~Asner} % 4684
% \author{H.~Atmacan} % 2538
% \author{V.~Aulchenko} % 8183
  \author{T.~Aushev} % 3747
  \author{V.~Aushev} % 2155
% \author{T.~Aziz} % 3523
% \author{V.~Babu} % 5623
% \author{S.~Bacher} % 2258
  \author{H.~Bae} % 10863
% \author{S.~Baehr} % 2515
% \author{S.~Bahinipati} % 2332
% \author{A.~M.~Bakich} % 2115
  \author{P.~Bambade} % 3003
  \author{Sw.~Banerjee} % 8603
% \author{S.~Bansal} % 5163
% \author{M.~Barrett} % 2180
% \author{G.~Batignani} % 6643
  \author{J.~Baudot} % 2562
  \author{M.~Bauer} % 9863
% \author{A.~Baur} % 5683
  \author{A.~Beaubien} % 6683
% \author{A.~Beaulieu} % 2444
  \author{J.~Becker} % 5403
  \author{P.~K.~Behera} % 4204
  \author{J.~V.~Bennett} % 2454
  \author{E.~Bernieri} % 4483
  \author{F.~U.~Bernlochner} % 2282
  \author{V.~Bertacchi} % 2212
  \author{M.~Bertemes} % 2595
  \author{E.~Bertholet} % 13163
  \author{M.~Bessner} % 3783
  \author{S.~Bettarini} % 2350
% \author{V.~Bhardwaj} % 2228
  \author{B.~Bhuyan} % 2097
  \author{F.~Bianchi} % 2564
  \author{T.~Bilka} % 2484
% \author{S.~Bilokin} % 3623
  \author{D.~Biswas} % 8703
% \author{A.~Bobrov} % 2294
  \author{D.~Bodrov} % 9643
  \author{A.~Bolz} % 15403
% \author{A.~Bondar} % 4643
% \author{G.~Bonvicini} % 2095
  \author{J.~Borah} % 7083
  \author{A.~Bozek} % 2303
  \author{M.~Bra\v{c}ko} % 2425
  \author{P.~Branchini} % 2577
% \author{N.~Braun} % 2436
  \author{R.~A.~Briere} % 2584
  \author{T.~E.~Browder} % 2560
% \author{D.~N.~Brown} % 8743
  \author{A.~Budano} % 2171
% \author{L.~Burmistrov} % 2111
  \author{S.~Bussino} % 5384
  \author{M.~Campajola} % 5223
  \author{L.~Cao} % 2099
  \author{G.~Casarosa} % 2491
  \author{C.~Cecchi} % 2433
% \author{D.~\v{C}ervenkov} % 2078
  \author{M.-C.~Chang} % 2827
% \author{P.~Chang} % 2542
% \author{R.~Cheaib} % 2208
  \author{P.~Cheema} % 15264
  \author{V.~Chekelian} % 2167
% \author{C.~Chen} % 12803
% \author{Y.~Q.~Chen} % 2576
  \author{Y.~Q.~Chen} % 16264
% \author{Y.-T.~Chen} % 2884
% \author{B.~G.~Cheon} % 2173
  \author{K.~Chilikin} % 2308
  \author{K.~Chirapatpimol} % 10803
  \author{H.-E.~Cho} % 2182
  \author{K.~Cho} % 2516
  \author{S.-J.~Cho} % 2723
  \author{S.-K.~Choi} % 2364
  \author{S.~Choudhury} % 2206
  \author{D.~Cinabro} % 2092
  \author{L.~Corona} % 3944
% \author{L.~M.~Cremaldi} % 2276
  \author{S.~Cunliffe} % 2272
% \author{T.~Czank} % 2254
  \author{S.~Das} % 9163
% \author{N.~Dash} % 2601
  \author{F.~Dattola} % 3745
  \author{E.~De~La~Cruz-Burelo} % 2359
  \author{S.~A.~De~La~Motte} % 2128
  \author{G.~de~Marino} % 8364
  \author{G.~De~Nardo} % 2459
  \author{M.~De~Nuccio} % 2610
  \author{G.~De~Pietro} % 2528
  \author{R.~de~Sangro} % 2524
% \author{B.~Deschamps} % 2671
  \author{M.~Destefanis} % 2594
  \author{S.~Dey} % 5023
  \author{A.~De~Yta-Hernandez} % 2104
  \author{R.~Dhamija} % 9465
  \author{A.~Di~Canto} % 10963
  \author{F.~Di~Capua} % 2065
% \author{S.~Di~Carlo} % 2079
  \author{J.~Dingfelder} % 2151
  \author{Z.~Dole\v{z}al} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez} % 2191
  \author{T.~V.~Dong} % 2215
  \author{M.~Dorigo} % 12543
  \author{K.~Dort} % 5583
% \author{D.~Dossett} % 2574
  \author{S.~Dreyer} % 12823
  \author{S.~Dubey} % 11063
% \author{S.~Duell} % 2344
  \author{G.~Dujany} % 9703
  \author{P.~Ecker} % 5563
% \author{S.~Eidelman} % 4984
  \author{M.~Eliachevitch} % 2725
 \author{D.~Epifanov} % 2551
  \author{P.~Feichtinger} % 9843
  \author{T.~Ferber} % 2482
  \author{D.~Ferlewicz} % 2073
  \author{T.~Fillinger} % 9803
% \author{C.~Finck} % 15803
  \author{G.~Finocchiaro} % 2400
% \author{P.~Fischer} % 2141
% \author{K.~Flood} % 12103
  \author{A.~Fodor} % 2312
  \author{F.~Forti} % 2432
% \author{A.~Frey} % 2150
% \author{M.~Friedl} % 2442
  \author{B.~G.~Fulsom} % 2563
% \author{M.~Gabriel} % 2443
% \author{A.~Gabrielli} % 13523
% \author{N.~Gabyshev} % 2510
  \author{E.~Ganiev} % 4623
% \author{M.~Garcia-Hernandez} % 4823
% \author{R.~Garg} % 2213
% \author{A.~Garmash} % 2161
  \author{V.~Gaur} % 2413
  \author{A.~Gaz} % 2181
% \author{U.~Gebauer} % 2174
  \author{A.~Gellrich} % 2480
% \author{J.~Gemmler} % 2321
% \author{T.~Ge{\ss}ler} % 2121
  \author{G.~Ghevondyan} % 9445
% \author{G.~Giakoustidis} % 13723
  \author{R.~Giordano} % 2103
  \author{A.~Giri} % 2106
  \author{A.~Glazov} % 2473
  \author{B.~Gobbo} % 2109
  \author{R.~Godang} % 2449
  \author{P.~Goldenzweig} % 2345
% \author{B.~Golob} % 3703
% \author{P.~Gomis} % 2354
% \author{G.~Gong} % 2727
% \author{P.~Grace} % 9563
  \author{W.~Gradl} % 2570
  \author{S.~Granderath} % 8383
  \author{E.~Graziani} % 2342
  \author{D.~Greenwald} % 2686
% \author{Z.~Gruberov\'{a}} % 8824
  \author{T.~Gu} % 14283
  \author{Y.~Guan} % 2514
  \author{K.~Gudkova} % 10504
  \author{J.~Guilliams} % 13543
% \author{C.~Hadjivasiliou} % 9503
% \author{S.~Halder} % 4743
% \author{K.~Hara} % 2462
% \author{T.~Hara} % 2523
% \author{O.~Hartbrich} % 2158
  \author{K.~Hayasaka} % 2330
  \author{H.~Hayashii} % 2455
  \author{S.~Hazra} % 7663
  \author{C.~Hearty} % 2450
% \author{M.~T.~Hedges} % 2265
  \author{I.~Heredia~de~la~Cruz} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva} % 2466
  \author{A.~Hershenhorn} % 2552
  \author{T.~Higuchi} % 2485
  \author{E.~C.~Hill} % 7823
  \author{H.~Hirata} % 2070
% \author{M.~Hoek} % 2101
  \author{M.~Hohmann} % 2077
% \author{S.~Hollitt} % 2557
% \author{T.~Hotta} % 2084
  \author{C.-L.~Hsu} % 2299
% \author{K.~Huang} % 2389
% \author{T.~Humair} % 10643
  \author{T.~Iijima} % 2446
  \author{K.~Inami} % 2323
  \author{G.~Inguglia} % 2500
  \author{N.~Ipsita} % 12223
% \author{J.~Irakkathil~Jabbar} % 7343
  \author{A.~Ishikawa} % 2281
  \author{S.~Ito} % 17463
 \author{R.~Itoh} % 2487
  \author{M.~Iwasaki} % 2360
% \author{Y.~Iwasaki} % 2229
% \author{S.~Iwata} % 4323
  \author{P.~Jackson} % 2255
  \author{W.~W.~Jacobs} % 2322
  \author{D.~E.~Jaffe} % 3663
  \author{E.-J.~Jang} % 6744
% \author{M.~Jeandron} % 2806
% \author{H.~B.~Jeon} % 2170
% \author{Q.~P.~Ji} % 16243
  \author{S.~Jia} % 2457
  \author{Y.~Jin} % 2105
% \author{C.~Joo} % 3525
  \author{K.~K.~Joo} % 4224
  \author{H.~Junkerkalefeld} % 12963
% \author{I.~Kadenko} % 3843
% \author{J.~Kahn} % 2448
% \author{H.~Kakuno} % 2391
% \author{M.~Kaleta} % 5603
  \author{A.~B.~Kaliyar} % 7344
% \author{J.~Kandra} % 2541
  \author{K.~H.~Kang} % 2283
% \author{S.~Kang} % 12683
% \author{P.~Kapusta} % 6663
  \author{R.~Karl} % 10923
  \author{G.~Karyan} % 2550
% \author{Y.~Kato} % 2549
% \author{H.~Kawai} % 4344
% \author{T.~Kawasaki} % 4363
% \author{C.~Ketter} % 2236
% \author{H.~Kichimi} % 2233
  \author{C.~Kiesling} % 2168
  \author{C.-H.~Kim} % 2358
  \author{D.~Y.~Kim} % 2315
% \author{H.~J.~Kim} % 4863
  \author{K.-H.~Kim} % 2118
% \author{K.~Kim} % 2409
% \author{S.-H.~Kim} % 2428
  \author{Y.-K.~Kim} % 2379
% \author{Y.~Kim} % 2403
% \author{T.~D.~Kimmel} % 2241
  \author{H.~Kindo} % 2195
  \author{K.~Kinoshita} % 2318
% \author{C.~Kleinwort} % 2499
% \author{B.~Knysh} % 8883
  \author{P.~Kody\v{s}} % 2407
  \author{T.~Koga} % 6963
  \author{S.~Kohani} % 9143
  \author{K.~Kojima} % 6363
% \author{I.~Komarov} % 2210
  \author{T.~Konno} % 2490
  \author{A.~Korobov} % 4185
  \author{S.~Korpar} % 2475
% \author{E.~Kou} % 3765
% \author{N.~Kovalchuk} % 6964
  \author{E.~Kovalenko} % 3884
  \author{R.~Kowalewski} % 2293
  \author{T.~M.~G.~Kraetzschmar} % 7543
% \author{F.~Krinner} % 9383
  \author{P.~Kri\v{z}an} % 2474
% \author{R.~Kroeger} % 2242
% \author{J.~F.~Krohn} % 2502
  \author{P.~Krokovny} % 2575
% \author{H.~Kr\"uger} % 2290
% \author{W.~Kuehn} % 2534
% \author{T.~Kuhr} % 2486
  \author{J.~Kumar} % 6464
% \author{M.~Kumar} % 2744
% \author{R.~Kumar} % 2189
  \author{K.~Kumara} % 2257
% \author{T.~Kumita} % 4083
  \author{T.~Kunigo} % 10104
% \author{M.~K\"{u}nzel} % 2139
% \author{S.~Kurz} % 9363
  \author{A.~Kuzmin} % 2520
% \author{P.~Kvasni\v{c}ka} % 2184
  \author{Y.-J.~Kwon} % 2231
  \author{S.~Lacaprara} % 2447
% \author{Y.-T.~Lai} % 2066
% \author{C.~La~Licata} % 2348
% \author{K.~Lalwani} % 2142
  \author{T.~Lam} % 2729
  \author{L.~Lanceri} % 2540
  \author{J.~S.~Lange} % 2277
  \author{M.~Laurenza} % 10223
  \author{K.~Lautenbach} % 2102
% \author{P.~J.~Laycock} % 7683
  \author{R.~Leboucher} % 14083
% \author{F.~R.~Le~Diberder} % 3267
% \author{I.-S.~Lee} % 2422
% \author{S.~C.~Lee} % 2544
% \author{P.~Leitl} % 2414
% \author{D.~Levit} % 2507
% \author{P.~M.~Lewis} % 2582
  \author{C.~Li} % 2325
  \author{L.~K.~Li} % 3263
% \author{S.~X.~Li} % 2377
% \author{Y.~B.~Li} % 2573
  \author{J.~Libby} % 2262
  \author{K.~Lieret} % 2268
% \author{J.~Lin} % 2401
  \author{Z.~Liptak} % 3565
  \author{Q.~Y.~Liu} % 7045
% \author{Z.~A.~Liu} % 3283
  \author{D.~Liventsev} % 2578
  \author{S.~Longo} % 2396
% \author{A.~Loos} % 2356
  \author{A.~Lozar} % 12423
% \author{P.~Lu} % 2148
  \author{T.~Lueck} % 2406
% \author{F.~Luetticke} % 2533
% \author{T.~Luo} % 3268
  \author{C.~Lyu} % 12484
% \author{C.~MacQueen} % 2585
  \author{M.~Maggiora} % 5343
  \author{R.~Maiti} % 12043
% \author{S.~Maity} % 2985
  \author{R.~Manfredi} % 10303
  \author{E.~Manoni} % 2305
% \author{A.~Manthei} % 15023
  \author{S.~Marcello} % 4223
  \author{C.~Marinas} % 2133
% \author{L.~Martel} % 13503
  \author{A.~Martini} % 2336
  \author{T.~Martinov} % 19463
  \author{L.~Massaccesi} % 16323
  \author{M.~Masuda} % 2238
% \author{T.~Matsuda} % 5543
% \author{K.~Matsuoka} % 2316
% \author{D.~Matvienko} % 2351
  \author{S.~K.~Maurya} % 9763
  \author{J.~A.~McKenna} % 2392
% \author{J.~McNeil} % 2382
% \author{F.~Meggendorfer} % 7103
  \author{F.~Meier} % 3103
  \author{M.~Merola} % 2456
  \author{F.~Metzner} % 2296
  \author{M.~Milesi} % 5443
  \author{C.~Miller} % 2273
  \author{K.~Miyabayashi} % 2327
% \author{H.~Miyake} % 2452
% \author{H.~Miyata} % 2071
  \author{R.~Mizuk} % 2483
% \author{K.~Azmi} % 2506
% \author{G.~B.~Mohanty} % 2278
  \author{N.~Molina-Gonzalez} % 8004
  \author{S.~Moneta} % 13303
% \author{H.~Moon} % 2304
% \author{T.~Moon} % 2397
% \author{J.~A.~Mora~Grimaldo} % 4403
% \author{T.~Morii} % 3543
  \author{H.-G.~Moser} % 2120
  \author{M.~Mrvar} % 2527
% \author{F.~J.~M\"{u}ller} % 2123
% \author{Th.~Muller} % 2165
% \author{G.~Muroyama} % 2093
% \author{C.~Murphy} % 12403
  \author{R.~Mussa} % 2372
  \author{I.~Nakamura} % 3463
% \author{K.~R.~Nakamura} % 2417
% \author{E.~Nakano} % 2554
  \author{M.~Nakao} % 2498
  \author{H.~Nakayama} % 2232
% \author{H.~Nakazawa} % 2335
  \author{Y.~Nakazawa} % 17383
  \author{A.~Narimani~Charan} % 10143
  \author{M.~Naruki} % 4583
% \author{D.~Narwal} % 7223
  \author{Z.~Natkaniec} % 3923
  \author{A.~Natochii} % 12063
  \author{L.~Nayak} % 9464
  \author{M.~Nayak} % 2371
  \author{G.~Nazaryan} % 9523
% \author{D.~Neverov} % 2075
% \author{C.~Niebuhr} % 2477
% \author{M.~Niiyama} % 2063
% \author{J.~Ninkovic} % 2386
  \author{N.~K.~Nisar} % 2522
% \author{S.~Nishida} % 2571
% \author{K.~Nishimura} % 3063
% \author{M.~H.~A.~Nouxman} % 2470
% \author{K.~Ogawa} % 2430
  \author{S.~Ogawa} % 6263
% \author{S.~L.~Olsen} % 4563
% \author{Y.~Onishchuk} % 2157
  \author{H.~Ono} % 2160
  \author{Y.~Onuki} % 2331
% \author{P.~Oskin} % 9623
% \author{F.~Otani} % 16244
  \author{E.~R.~Oxford} % 6943
% \author{H.~Ozaki} % 2984
% \author{P.~Pakhlov} % 2221
% \author{G.~Pakhlova} % 2188
  \author{A.~Paladino} % 2435
% \author{T.~Pang} % 2114
  \author{A.~Panta} % 7943
  \author{E.~Paoloni} % 2488
  \author{S.~Pardi} % 2532
% \author{K.~Parham} % 10684
  \author{H.~Park} % 2284
  \author{S.-H.~Park} % 2509
% \author{B.~Paschen} % 2159
  \author{A.~Passeri} % 2116
% \author{A.~Pathak} % 8723
% \author{S.~Patra} % 3123
  \author{S.~Paul} % 2131
  \author{T.~K.~Pedlar} % 2421
  \author{I.~Peruzzi} % 2253
  \author{R.~Peschke} % 7123
  \author{R.~Pestotnik} % 2476
% \author{F.~Pham} % 2963
  \author{M.~Piccolo} % 2147
  \author{L.~E.~Piilonen} % 2346
% \author{G.~Pinna~Angioni} % 13363
  \author{P.~L.~M.~Podesta-Lerma} % 2266
  \author{T.~Podobnik} % 11223
  \author{S.~Pokharel} % 12283
  \author{L.~Polat} % 9783
% \author{V.~Popov} % 2096
  \author{C.~Praz} % 2726
  \author{S.~Prell} % 12743
  \author{E.~Prencipe} % 2219
  \author{M.~T.~Prim} % 2501
% \author{M.~V.~Purohit} % 2196
  \author{H.~Purwar} % 12363
  \author{N.~Rad} % 11683
  \author{P.~Rados} % 7383
  \author{S.~Raiz} % 13003
  \author{A.~Ramirez~Morales} % 13724
% \author{R.~Rasheed} % 3643
% \author{N.~Rauls} % 11603
  \author{M.~Reif} % 8043
  \author{S.~Reiter} % 2248
  \author{M.~Remnev} % 2785
  \author{I.~Ripp-Baudot} % 2469
% \author{M.~Ritter} % 2580
% \author{M.~Ritzert} % 2526
  \author{G.~Rizzo} % 2579
% \author{L.~B.~Rizzuto} % 3746
  \author{S.~H.~Robertson} % 2471
% \author{D.~Rodr\'{i}guez~P\'{e}rez} % 2176
  \author{J.~M.~Roney} % 2244
% \author{C.~Rosenfeld} % 2082
  \author{A.~Rostomyan} % 2481
  \author{N.~Rout} % 2965
% \author{M.~Rozanska} % 2205
  \author{G.~Russo} % 2388
% \author{D.~Sahoo} % 2110
% \author{Y.~Sakai} % 2175
  \author{D.~A.~Sanders} % 2458
 \author{S.~Sandilya} % 2286
  \author{A.~Sangal} % 2384
% \author{L.~Santelj} % 2185
% \author{P.~Sartori} % 4523
  \author{Y.~Sato} % 5243
  \author{V.~Savinov} % 2292
  \author{B.~Scavino} % 2518
% \author{M.~Schnepf} % 15683
% \author{M.~Schram} % 2306
% \author{H.~Schreeck} % 2434
  \author{J.~Schueler} % 2824
  \author{C.~Schwanda} % 2108
  \author{A.~J.~Schwartz} % 2162
  \author{B.~Schwenker} % 2405
% \author{M.~Schwickardi} % 14743
  \author{Y.~Seino} % 2517
  \author{A.~Selce} % 9043
  \author{K.~Senyo} % 2987
% \author{I.~S.~Seong} % 2572
  \author{J.~Serrano} % 12124
  \author{M.~E.~Sevior} % 2328
  \author{C.~Sfienti} % 2214
% \author{C.~Sharma} % 11584
% \author{V.~Shebalin} % 2339
  \author{C.~P.~Shen} % 2464
  \author{X.~D.~Shi} % 18843
% \author{H.~Shibuya} % 2234
  \author{T.~Shillington} % 7983
% \author{T.~Shimasaki} % 16263
% \author{J.-G.~Shiu} % 2412
% \author{B.~Shwartz} % 2122
  \author{A.~Sibidanov} % 2419
% \author{F.~Simon} % 2164
  \author{J.~B.~Singh} % 2903
% \author{S.~Skambraks} % 2394
  \author{J.~Skorupa} % 12523
% \author{K.~Smith} % 2243
  \author{R.~J.~Sobie} % 2472
  \author{A.~Soffer} % 2217
% \author{A.~Sokolov} % 2521
% \author{Y.~Soloviev} % 2479
  \author{E.~Solovieva} % 2398
  \author{S.~Spataro} % 2117
  \author{B.~Spruck} % 2493
  \author{M.~Stari\v{c}} % 2326
  \author{S.~Stefkova} % 8783
  \author{Z.~S.~Stottler} % 2267
  \author{R.~Stroili} % 2465
  \author{J.~Strube} % 2451
% \author{J.~Stypula} % 2368
% \author{Y.~Sue} % 2085
% \author{R.~Sugiura} % 4644
  \author{M.~Sumihama} % 4243
  \author{K.~Sumisawa} % 2583
% \author{T.~Sumiyoshi} % 4184
  \author{W.~Sutcliffe} % 3784
  \author{S.~Y.~Suzuki} % 2496
  \author{H.~Svidras} % 11783
% \author{M.~Tabata} % 2986
% \author{M.~Takahashi} % 2467
  \author{M.~Takizawa} % 2437
  \author{U.~Tamponi} % 2366
% \author{S.~Tanaka} % 2530
  \author{K.~Tanida} % 3803
  \author{H.~Tanigawa} % 2237
% \author{N.~Taniguchi} % 2285
% \author{Y.~Tao} % 2362
% \author{P.~Taras} % 2202
  \author{F.~Tenchini} % 2546
  \author{A.~Thaller} % 16044
  \author{R.~Tiwary} % 10403
  \author{D.~Tonelli} % 4564
  \author{E.~Torassa} % 2556
  \author{N.~Toutounji} % 2263
  \author{K.~Trabelsi} % 2369
% \author{I.~Tsaklidis} % 13443
% \author{T.~Tsuboyama} % 2361
% \author{N.~Tsuzuki} % 2352
  \author{M.~Uchida} % 2370
  \author{I.~Ueda} % 2519
% \author{S.~Uehara} % 2586
  \author{Y.~Uematsu} % 5883
% \author{T.~Ueno} % 4364
  \author{T.~Uglov} % 2252
  \author{K.~Unger} % 9463
  \author{Y.~Unno} % 2420
  \author{K.~Uno} % 14963
  \author{S.~Uno} % 2149
% \author{P.~Urquijo} % 2302
  \author{Y.~Ushiroda} % 2317
% \author{Y.~V.~Usov} % 5003
  \author{S.~E.~Vahsen} % 2251
  \author{R.~van~Tonder} % 2706
  \author{G.~S.~Varner} % 2119
  \author{K.~E.~Varvell} % 2545
  \author{A.~Vinokurova} % 2289
  \author{L.~Vitale} % 2415
  \author{V.~Vobbilisetti} % 7364
% \author{V.~Vorobyev} % 2298
% \author{A.~Vossen} % 2249
% \author{B.~Wach} % 8203
% \author{E.~Waheed} % 2226
  \author{H.~M.~Wakeling} % 3664
% \author{K.~Wan} % 2591
% \author{W.~Wan~Abdullah} % 2280
% \author{B.~Wang} % 2569
% \author{C.~H.~Wang} % 2224
  \author{E.~Wang} % 10983
  \author{M.-Z.~Wang} % 2074
  \author{X.~L.~Wang} % 2076
  \author{A.~Warburton} % 2347
  \author{M.~Watanabe} % 2309
  \author{S.~Watanuki} % 6843
% \author{J.~Webb} % 2423
% \author{S.~Wehle} % 2489
  \author{M.~Welsch} % 7023
% \author{O.~Werbycka} % 6123
  \author{C.~Wessel} % 2100
% \author{J.~Wiechczynski} % 2604
% \author{P.~Wieduwilt} % 2343
% \author{H.~Windel} % 2081
  \author{E.~Won} % 2410
% \author{L.~J.~Wu} % 2704
% \author{X.~P.~Xu} % 4923
  \author{B.~D.~Yabsley} % 3645
  \author{S.~Yamada} % 2492
  \author{W.~Yan} % 2094
  \author{S.~B.~Yang} % 2374
  \author{H.~Ye} % 2537
  \author{J.~Yelton} % 2067
  \author{J.~H.~Yin} % 2365
% \author{M.~Yonenaga} % 2411
  \author{Y.~M.~Yook} % 2453
  \author{K.~Yoshihara} % 12663
% \author{T.~Yoshinobu} % 2429
  \author{C.~Z.~Yuan} % 2088
% \author{Y.~Yusa} % 2357
  \author{L.~Zani} % 2529
% \author{Y.~Zhai} % 12703
% \author{J.~Z.~Zhang} % 2349
% \author{Y.~Zhang} % 2607
  \author{Y.~Zhang} % 3303
% \author{Z.~Zhang} % 5363
 \author{V.~Zhilich} % 4703
% \author{J.~S.~Zhou} % 12463
  \author{Q.~D.~Zhou} % 7323
  \author{X.~Y.~Zhou} % 2380
  \author{V.~I.~Zhukova} % 2387
% \author{V.~Zhulanov} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k} % 13403
\collaboration{The Belle II Collaboration}


==> pub012.tex <==
%%% Paper:    Omega_c lifetime
%%% Journal:  Physical Review D (L)
%%% Contacts: A. Di Canto, N.K. Nisar
%%% ====================================================================
%%% Use \input{pub012} to insert this material into your latex file.
%%%\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
%%%\newcommand{\instBUAP}{Benemerita Universidad Autonoma de Puebla, Puebla 72570, Mexico}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
%%%\newcommand{\instChula}{Chulalongkorn University, Bangkok 10330, Thailand}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instRomaENEA}{ENEA Casaccia, I-00123 Roma, Italy}
%%%\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (SOKENDAI), Hayama 240-0193, Japan}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007, China}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
%%%\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081, China}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
%%%\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011, U.S.A.}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instMainz}{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
%%%\newcommand{\instKennesaw}{Kennesaw State University, Kennesaw, Georgia 30144, U.S.A.}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLPI}{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991, Russian Federation}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
%%%\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
%%%\newcommand{\instNNU}{Nanjing Normal University, Nanjing 210023, China}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
%%%\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
%%%\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\newcommand{\instRIKEN}{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
%%%\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instKyiv}{Taras Shevchenko National Univ. of Kiev, Kiev, Ukraine}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
%%%\newcommand{\instECUTUM}{Excellence Cluster Universe, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
%%%\newcommand{\instNapoliUNIVA}{Dipartimento di Agraria, Universit\`{a} di Napoli Federico II, I-80055 Portici (NA), Italy}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
%%%\newcommand{\instRomaUNIV}{Universit\`{a} di Roma ``La Sapienza,'' I-00185 Roma, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
%%%\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instHeidelberg}{University of Heidelberg, 68131 Mannheim, Germany}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007, India}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
%%%\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
%%%\newcommand{\instZZU}{Zhengzhou University, Zhengzhou 450001, China}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instYerevan}
%%%\affiliation{\instBeihang}
%%%\affiliation{\instBUAP}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
%%%\affiliation{\instChiba}
\affiliation{\instChonnam}
%%%\affiliation{\instChula}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
\affiliation{\instRomaENEA}
%%%\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGoettingen}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
%%%\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHNU}
\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
%%%\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
%%%\affiliation{\instIISER}
%%%\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
%%%\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instISU}
\affiliation{\instJAEA}
\affiliation{\instMainz}
\affiliation{\instGiessen}
\affiliation{\instKarlsruhe}
%%%\affiliation{\instKennesaw}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLPI}
\affiliation{\instLNNU}
\affiliation{\instLMU}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instMPP}
%%%\affiliation{\instMPGHLL}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaIAR}
\affiliation{\instNagoyaKMI}
%%%\affiliation{\instNNU}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
%%%\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
%%%\affiliation{\instOkinawa}
%%%\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
%%%\affiliation{\instPeking}
%%%\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKEN}
\affiliation{\instXavier}
%%%\affiliation{\instSeoul}
%%%\affiliation{\instShandong}
\affiliation{\instSPU}
%%%\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instKyiv}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instECUTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
%%%\affiliation{\instTohoku}
\affiliation{\instTitech}
%%%\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
%%%\affiliation{\instNapoliUNIVA}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
%%%\affiliation{\instRomaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
%%%\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
%%%\affiliation{\instHeidelberg}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
%%%\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
%%%\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
%%%\affiliation{\instZZU}
  \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
% \author{K.~Adamczyk}\affiliation{\instLjubljanaJSI} % 2239
  \author{L.~Aggarwal}\affiliation{\instPanjab} % 10083
% \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{H.~Ahmed}\affiliation{\instXavier} % 11323
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2194
% \author{F.~Ameli}\affiliation{\instRomaINFN} % 4683
% \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
 \author{N.~Anh~Ky}\affiliation{\instIOP} % 2218
 \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
% \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
% \author{T.~Aziz}\affiliation{\instTata} % 3523
% \author{V.~Babu}\affiliation{\instIPHC} % 5623
% \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{H.~Bae}\affiliation{\instUTokyo} % 10863
% \author{S.~Baehr}\affiliation{\instKarlsruhe} % 2515
% \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
% \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
% \author{S.~Bansal}\affiliation{\instPanjab} % 5163
% \author{M.~Barrett}\affiliation{\instKEK} % 2180
% \author{G.~Batignani}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{M.~Bauer}\affiliation{\instKarlsruhe} % 9863
% \author{A.~Baur}\affiliation{\instDESY} % 5683
  \author{A.~Beaubien}\affiliation{\instVictoria} % 6683
% \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
  \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{V.~Bertacchi}\affiliation{\instCPPM} % 2212
  \author{M.~Bertemes}\affiliation{\instBNL} % 2595
  \author{E.~Bertholet}\affiliation{\instTelAviv} % 13163
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2350
% \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
% \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
% \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{D.~Bodrov}\affiliation{\instHSE}\affiliation{\instLPI} % 9643
  \author{A.~Bolz}\affiliation{\instDESY} % 15403
% \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
% \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{J.~Borah}\affiliation{\instIITGuwahati} % 7083
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
% \author{N.~Braun}\affiliation{\instKarlsruhe} % 2436
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
% \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
% \author{L.~Burmistrov}\affiliation{\instIJCLab} % 2111
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instDESY} % 2099
  \author{G.~Casarosa}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaINFN}\affiliation{\instPerugiaUNIV} % 2433
% \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
% \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
% \author{R.~Cheaib}\affiliation{\instDESY} % 2208
  \author{P.~Cheema}\affiliation{\instSydney} % 15264
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
% \author{C.~Chen}\affiliation{\instISU} % 12803
% \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
  \author{Y.~Q.~Chen}\affiliation{\instHUNNU} % 16264
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
% \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instLPI} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instCAU} % 2364
  \author{S.~Choudhury}\affiliation{\instISU} % 2206
  \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{L.~Corona}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 3944
% \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % 2254
  \author{S.~Das}\affiliation{\instMNITJaipur} % 9163
% \author{N.~Dash}\affiliation{\instIITMadras} % 2601
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{S.~A.~De~La~Motte}\affiliation{\instAdelaide} % 2128
  \author{G.~de~Marino}\affiliation{\instIJCLab} % 8364
  \author{G.~De~Nardo}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2459
  \author{M.~De~Nuccio}\affiliation{\instUBC} % 2610
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
% \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
  \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{R.~Dhamija}\affiliation{\instIITHyderabad} % 9465
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2065
% \author{S.~Di~Carlo}\affiliation{\instIJCLab} % 2079
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instITAR} % 2215
  \author{M.~Dorigo}\affiliation{\instTriesteINFN} % 12543
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
% \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dreyer}\affiliation{\instDESY} % 12823
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
% \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % 5563
% \author{S.~Eidelman}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 4984
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
 \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{P.~Feichtinger}\affiliation{\instHEPHYVienna} % 9843
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{T.~Fillinger}\affiliation{\instIPHC} % 9803
% \author{C.~Finck}\affiliation{\instIPHC} % 15803
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
% \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
% \author{K.~Flood}\affiliation{\instHawaii} % 12103
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2432
% \author{A.~Frey}\affiliation{\instGoettingen} % 2150
% \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
% \author{M.~Gabriel}\affiliation{\instMPP} % 2443
% \author{A.~Gabrielli}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13523
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instDESY} % 4623
% \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
% \author{R.~Garg}\affiliation{\instPanjab} % 2213
% \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{V.~Gaur}\affiliation{\instUPES} % 2413
  \author{A.~Gaz}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2181
% \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
% \author{J.~Gemmler}\affiliation{\instKarlsruhe} % 2321
% \author{T.~Ge{\ss}ler}\affiliation{\instGiessen} % 2121
  \author{G.~Ghevondyan}\affiliation{\instYerevan} % 9445
% \author{G.~Giakoustidis}\affiliation{\instBonn} % 13723
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
% \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI}\affiliation{\instNovaGorica} % 3703
% \author{P.~Gomis}\affiliation{\instIFIC} % 2354
% \author{G.~Gong}\affiliation{\instUSTC} % 2727
% \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
  \author{S.~Granderath}\affiliation{\instBonn} % 8383
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
% \author{Z.~Gruberov\'{a}}\affiliation{\instPrague} % 8824
  \author{T.~Gu}\affiliation{\instPittsburgh} % 14283
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % 10504
  \author{J.~Guilliams}\affiliation{\instMississippi} % 13543
% \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
% \author{S.~Halder}\affiliation{\instTata} % 4743
% \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
% \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
% \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{S.~Hazra}\affiliation{\instTata} % 7663
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
% \author{M.~T.~Hedges}\affiliation{\instBonn} % 2265
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instDESY} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
  \author{H.~Hirata}\affiliation{\instNagoya} % 2070
% \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
% \author{S.~Hollitt}\affiliation{\instAdelaide} % 2557
% \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
% \author{T.~Humair}\affiliation{\instMPP} % 10643
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instKEK}\affiliation{\instNagoyaKMI} % 2446
  \author{K.~Inami}\affiliation{\instNagoya}\affiliation{\instKEK} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % 12223
% \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{S.~Ito}\affiliation{\instKEK} % 17463
 \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % 2360
% \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instCAU} % 6744
% \author{M.~Jeandron}\affiliation{\instMississippi} % 2806
% \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
% \author{Q.~P.~Ji}\affiliation{\instHNU} % 16243
  \author{S.~Jia}\affiliation{\instFudan} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
% \author{C.~Joo}\affiliation{\instIPMU} % 3525
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{H.~Junkerkalefeld}\affiliation{\instBonn} % 12963
% \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
% \author{J.~Kahn}\affiliation{\instKarlsruhe} % 2448
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
% \author{M.~Kaleta}\affiliation{\instKrakow} % 5603
  \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % 7344
% \author{J.~Kandra}\affiliation{\instPrague} % 2541
  \author{K.~H.~Kang}\affiliation{\instIPMU} % 2283
% \author{S.~Kang}\affiliation{\instISU} % 12683
% \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{R.~Karl}\affiliation{\instDESY} % 10923
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
% \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
% \author{H.~Kawai}\affiliation{\instChiba} % 4344
% \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
% \author{C.~Ketter}\affiliation{\instHawaii} % 2236
% \author{H.~Kichimi}\affiliation{\instKEK} % 2233
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
% \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{K.-H.~Kim}\affiliation{\instKISTI} % 2118
% \author{K.~Kim}\affiliation{\instKoreaUnivKU} % 2409
% \author{S.-H.~Kim}\affiliation{\instSeoul} % 2428
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
% \author{Y.~Kim}\affiliation{\instKoreaUnivKU} % 2403
% \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
% \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
% \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{K.~Kojima}\affiliation{\instNagoya} % 6363
% \author{I.~Komarov}\affiliation{\instDESY} % 2210
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % 4185
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
% \author{N.~Kovalchuk}\affiliation{\instDESY} % 6964
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % 3884
  \author{R.~Kowalewski}\affiliation{\instVictoria} % 2293
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
% \author{F.~Krinner}\affiliation{\instMPP} % 9383
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
% \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
% \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
% \author{H.~Kr\"uger}\affiliation{\instBonn} % 2290
% \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
% \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
% \author{M.~Kumar}\affiliation{\instMNITJaipur} % 2744
% \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instMississippi} % 2257
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
% \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
% \author{S.~Kurz}\affiliation{\instDESY} % 9363
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
% \author{Y.-T.~Lai}\affiliation{\instIPMU} % 2066
% \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
% \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{T.~Lam}\affiliation{\instVPI} % 2729
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{M.~Laurenza}\affiliation{\instRomaTreINFN}\affiliation{\instRomaTreUNIV} % 10223
  \author{K.~Lautenbach}\affiliation{\instCPPM} % 2102
% \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{R.~Leboucher}\affiliation{\instCPPM} % 14083
% \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
% \author{I.-S.~Lee}\affiliation{\instHanyang} % 2422
% \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
% \author{P.~Leitl}\affiliation{\instMPP} % 2414
% \author{D.~Levit}\affiliation{\instKEK} % 2507
% \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
% \author{S.~X.~Li}\affiliation{\instFudan} % 2377
% \author{Y.~B.~Li}\affiliation{\instFudan} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{K.~Lieret}\affiliation{\instLMU} % 2268
% \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{Z.~Liptak}\affiliation{\instHiroshima} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
% \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instDESY} % 2396
% \author{A.~Loos}\affiliation{\instSCarolina} % 2356
  \author{A.~Lozar}\affiliation{\instLjubljanaJSI} % 12423
% \author{P.~Lu}\affiliation{\instNTUTaiwan} % 2148
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
% \author{F.~Luetticke}\affiliation{\instBonn} % 2533
% \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~Lyu}\affiliation{\instBonn} % 12484
% \author{C.~MacQueen}\affiliation{\instMelbourne} % 2585
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{R.~Maiti}\affiliation{\instHEPHYVienna} % 12043
% \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
% \author{A.~Manthei}\affiliation{\instBonn} % 15023
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
% \author{L.~Martel}\affiliation{\instIPHC} % 13503
  \author{A.~Martini}\affiliation{\instDESY} % 2336
  \author{T.~Martinov}\affiliation{\instDESY} % 19463
  \author{L.~Massaccesi}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 16323
  \author{M.~Masuda}\affiliation{\instRCNP}\affiliation{\instEri} % 2238
% \author{T.~Matsuda}\affiliation{\instUOM} % 5543
% \author{K.~Matsuoka}\affiliation{\instKEK}\affiliation{\instNagoya} % 2316
% \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU}\affiliation{\instLPI} % 2351
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % 9763
  \author{J.~A.~McKenna}\affiliation{\instUBC} % 2392
% \author{J.~McNeil}\affiliation{\instFlorida} % 2382
% \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliINFN}\affiliation{\instNapoliUNIV} % 2456
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % 2327
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
% \author{H.~Miyata}\affiliation{\instNiigata} % 2071
  \author{R.~Mizuk}\affiliation{\instLPI}\affiliation{\instHSE} % 2483
% \author{K.~Azmi}\affiliation{\instMalaya} % 2506
% \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{N.~Molina-Gonzalez}\affiliation{\instCinvestavIPN} % 8004
  \author{S.~Moneta}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 13303
% \author{H.~Moon}\affiliation{\instKoreaUnivKU} % 2304
% \author{T.~Moon}\affiliation{\instSeoul} % 2397
% \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
% \author{T.~Morii}\affiliation{\instIPMU} % 3543
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
% \author{F.~J.~M\"{u}ller}\affiliation{\instDESY} % 2123
% \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
% \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
% \author{C.~Murphy}\affiliation{\instIPMU} % 12403
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
% \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
  \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{Y.~Nakazawa}\affiliation{\instKEK} % 17383
  \author{A.~Narimani~Charan}\affiliation{\instDESY} % 10143
  \author{M.~Naruki}\affiliation{\instKyotoU} % 4583
% \author{D.~Narwal}\affiliation{\instIITGuwahati} % 7223
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{L.~Nayak}\affiliation{\instIITHyderabad} % 9464
  \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
% \author{D.~Neverov}\affiliation{\instNagoya} % 2075
% \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
% \author{M.~Niiyama}\affiliation{\instKSU} % 2063
% \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
% \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2571
% \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
% \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
% \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
% \author{S.~L.~Olsen}\affiliation{\instCAU} % 4563
% \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
% \author{P.~Oskin}\affiliation{\instLPI} % 9623
% \author{F.~Otani}\affiliation{\instUTokyo} % 16244
  \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
% \author{P.~Pakhlov}\affiliation{\instLPI} % 2221
% \author{G.~Pakhlova}\affiliation{\instHSE}\affiliation{\instLPI} % 2188
  \author{A.~Paladino}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2435
% \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
% \author{K.~Parham}\affiliation{\instDuke} % 10684
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{S.-H.~Park}\affiliation{\instKEK} % 2509
% \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
% \author{A.~Pathak}\affiliation{\instLouisville} % 8723
% \author{S.~Patra}\affiliation{\instIISER} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
% \author{F.~Pham}\affiliation{\instMelbourne} % 2963
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
% \author{G.~Pinna~Angioni}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 13363
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{T.~Podobnik}\affiliation{\instLjubljanaJSI} % 11223
  \author{S.~Pokharel}\affiliation{\instMississippi} % 12283
  \author{L.~Polat}\affiliation{\instCPPM} % 9783
% \author{V.~Popov}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instDESY} % 2726
  \author{S.~Prell}\affiliation{\instISU} % 12743
  \author{E.~Prencipe}\affiliation{\instGiessen} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
% \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{H.~Purwar}\affiliation{\instHawaii} % 12363
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instHEPHYVienna} % 7383
  \author{S.~Raiz}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 13003
  \author{A.~Ramirez~Morales}\affiliation{\instKyungpook} % 13724
% \author{R.~Rasheed}\affiliation{\instIPHC} % 3643
% \author{N.~Rauls}\affiliation{\instGoettingen} % 11603
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
% \author{M.~Ritter}\affiliation{\instLMU} % 2580
% \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaINFN}\affiliation{\instPisaUNIV} % 2579
% \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
% \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
% \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2965
% \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
% \author{D.~Sahoo}\affiliation{\instISU} % 2110
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
 \author{S.~Sandilya}\affiliation{\instIITHyderabad} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
% \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
% \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{Y.~Sato}\affiliation{\instKEK} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instMainz} % 2518
% \author{M.~Schnepf}\affiliation{\instKarlsruhe} % 15683
% \author{M.~Schram}\affiliation{\instPNNL} % 2306
% \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
  \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
  \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
% \author{M.~Schwickardi}\affiliation{\instGoettingen} % 14743
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaTreINFN}\affiliation{\instRomaENEA} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
% \author{I.~S.~Seong}\affiliation{\instHawaii} % 2572
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
% \author{C.~Sharma}\affiliation{\instMNITJaipur} % 11584
% \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instFudan} % 2464
  \author{X.~D.~Shi}\affiliation{\instKEK} % 18843
% \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{T.~Shillington}\affiliation{\instMcGill} % 7983
% \author{T.~Shimasaki}\affiliation{\instUTokyo} % 16263
% \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
% \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instHawaii} % 2419
% \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
% \author{S.~Skambraks}\affiliation{\instKarlsruhe} % 2394
  \author{J.~Skorupa}\affiliation{\instMPP} % 12523
% \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
% \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
% \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instLPI} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoINFN}\affiliation{\instTorinoUNIV} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{S.~Stefkova}\affiliation{\instKarlsruhe} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaINFN}\affiliation{\instPadovaUNIV} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
% \author{J.~Stypula}\affiliation{\instKrakow} % 2368
% \author{Y.~Sue}\affiliation{\instNagoya} % 2085
% \author{R.~Sugiura}\affiliation{\instUTokyo} % 4644
  \author{M.~Sumihama}\affiliation{\instRCNP}\affiliation{\instGifu} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2583
% \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % 4184
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
% \author{M.~Tabata}\affiliation{\instChiba} % 2986
% \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
  \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
% \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
% \author{Y.~Tao}\affiliation{\instFlorida} % 2362
% \author{P.~Taras}\affiliation{\instMontreal} % 2202
  \author{F.~Tenchini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2546
  \author{A.~Thaller}\affiliation{\instCPPM} % 16044
  \author{R.~Tiwary}\affiliation{\instTata} % 10403
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{N.~Toutounji}\affiliation{\instSydney} % 2263
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
% \author{I.~Tsaklidis}\affiliation{\instBonn} % 13443
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{Y.~Uematsu}\affiliation{\instUTokyo} % 5883
% \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instLPI}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{K.~Uno}\affiliation{\instNiigata} % 14963
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
% \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instUTokyo}\affiliation{\instSOKENDAI} % 2317
% \author{Y.~V.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instMcGill} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vobbilisetti}\affiliation{\instIJCLab} % 7364
% \author{V.~Vorobyev}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2298
% \author{A.~Vossen}\affiliation{\instDuke} % 2249
% \author{B.~Wach}\affiliation{\instMPP} % 8203
% \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
% \author{K.~Wan}\affiliation{\instUTokyo} % 2591
% \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
% \author{B.~Wang}\affiliation{\instMPP} % 2569
% \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{E.~Wang}\affiliation{\instPittsburgh} % 10983
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instYonsei} % 6843
% \author{J.~Webb}\affiliation{\instMelbourne} % 2423
% \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
% \author{O.~Werbycka}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 6123
  \author{C.~Wessel}\affiliation{\instBonn} % 2100
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % 2604
% \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
% \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % 2410
% \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
% \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % 2374
  \author{H.~Ye}\affiliation{\instDESY} % 2537
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{J.~H.~Yin}\affiliation{\instKoreaUnivKU} % 2365
% \author{M.~Yonenaga}\affiliation{\instTokyoMetropolitan} % 2411
  \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{K.~Yoshihara}\affiliation{\instNagoya} % 12663
% \author{T.~Yoshinobu}\affiliation{\instNiigata} % 2429
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
% \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instCPPM} % 2529
% \author{Y.~Zhai}\affiliation{\instISU} % 12703
% \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
% \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Y.~Zhang}\affiliation{\instFudan} % 3303
% \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
 \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
% \author{J.~S.~Zhou}\affiliation{\instFudan} % 12463
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaIAR}\affiliation{\instNagoyaKMI} % 7323
  \author{X.~Y.~Zhou}\affiliation{\instLNNU} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLPI} % 2387
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k}\affiliation{\instPrague} % 13403
\collaboration{The Belle II Collaboration}


==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa

